A Survey and Empirical Evaluation of Parallel Deep Learning Frameworks

The field of deep learning has witnessed a remarkable shift towards extremely compute- and memory-intensive neural networks. These newer larger models have enabled researchers to advance state-of-the-art tools across a variety of fields. This phenomenon has spurred the development of algorithms for distributed training of neural networks over a larger number of hardware accelerators. In this paper, we discuss and compare current state-of-the-art frameworks for large scale distributed deep learning. First, we survey current practices in distributed learning and identify the different types of parallelism used. Then, we present empirical results comparing their performance on large image and language training tasks. Additionally, we address their statistical efficiency and memory consumption behavior. Based on our results, we discuss algorithmic and implementation portions of each framework which hinder performance.

==> survey-hybrid.tex <==

\suggest{I dont understand this section, What are generalizing techniques?}
Advancements in data parallelism continue to provide performance improvements 
even at the supercomputing level. Ying et al. \cite{ying2018image} employ several data parallelism 
techniques to a 1024 TPU supercomputing and train ResNet-50 on Imagenet  to 76.3\% 
accuracy in only 2.2 minutes. Researchers at the Summit Supercomputer \cite{summit2019} provide 
configuration guidelines to deploy any deep learning model at a supercomputing scale.

These same techniques are often used to create scalable hybrid-parallel models. 
Oyama et al. \cite{oyama2020case} incorporate data parallelism with spatially partitioned 
3-dimension data to realize strong scaling and accuracy improvements in 3D CNN. 
FlexFlow \cite{jia2018data} utilizes data parallelism’s efficiency for compute-intensive 
operations when searching for the best hybrid-parallel strategy for a given hardware.


==> tables/empirical-frameworks.tex <==
\begin{table*}[t]
    \caption{Summary of Literature Reviewed}
    \label{tab:emp-frameworks}
    \begin{tabular}{@{}llllll@{}}
    \toprule
    Framework & Type of Parallelism & Neural Networks & commit  \\ \midrule
    Pytorch DDP & Data Parallelism & VGG16, Resnet50, GPT2-small, GPT2-medium &  1234  \\ \midrule
    ZeRO & Data Parallelism & VGG16, Resnet50, GPT2-small, GPT2-medium &  1234  \\ \midrule
    MegatronLM & Intra-layer parallelism & GPT2-small, GPT2-medium &  1234  \\ \midrule
    Torchgpipe & Inter-layer parallelism & VGG16, Resnet50, GPT2-small, GPT2-medium &  1234  \\ \midrule
    Pipedream & Inter-layer parallelism & VGG16, GPT2-small, GPT2-medium &  1234  \\ \bottomrule
    \end{tabular}
\end{table*}

==> tables/exp-setup.tex <==
\begin{table*}[t]
    \caption{Metrics}
    \label{tab:metrics}
    \begin{tabular}{@{}llllll@{}}
    \toprule
    Metric & Machines & Neural Networks \\ \midrule
    Epoch execution times & ThetaGPU, Lassen and Vulcan & VGG16, ResNet50, GPT2-small, GPT2-medium  \\ \midrule
    Statistical efficiency & ThetaGPU & VGG16, GPT2-small \\ \midrule
    Memory utilisation & ThetaGPU & GPT2-medium \\ \bottomrule
    \end{tabular}
\end{table*}

==> tables/network-parameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\caption{Networks and Parameters}
\label{tab:network-parameters}
\begin{tabular}{@{}llllll@{}}
\toprule
Network           & Dataset      & \begin{tabular}[c]{@{}l@{}}Batch\\ Size\end{tabular} & Optimizer & \begin{tabular}[c]{@{}l@{}}Learning\\ Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}LR\\ Schedule\end{tabular} \\ \midrule
VGG-16             & Imagenet     & 64                                                   & SGD       & 0.01                                                    & \checkmark                                            \\ \midrule
ResNet-50         & Imagenet     & 128                                                  & LARS      & 5.0                                                     & \checkmark                                            \\ \midrule
GPT2-small & WikiText-103 & 32                                                   & LAMB      &                                                         &                                                       \\ \midrule
GPT2-medium & WikiText-103 & 32                                                   & LAMB      &                                                         &                                                       \\ \bottomrule
\end{tabular}
\end{table*}


==> tables/stopping-conditions.tex <==
\begin{table}[]
\caption{Experiments}
\label{tab:experiment-desc}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Model} & \textbf{Dataset} & \textbf{Stopping Condition} \\ \hline
VGG-16         & Imagenet         & 68\% accuracy               \\ \hline
ResNet-50      & Imagenet         & 75.9\% accuracy             \\ \hline
BERT           & Wikipedia        & N/A                         \\ \hline
GPT-2          & Wikipedia        & N/A                         \\ \hline
\end{tabular}
\end{table}

